Click to Grasp: Zero-Shot Precise Manipulation via Visual Diffusion Descriptors

Precise manipulation that is generalizable across scenes and objects remains a persistent challenge in robotics. Current approaches for this task heavily depend on having a significant number of training instances to handle objects with pronounced visual and/or geometric part ambiguities. Our work explores the grounding of fine-grained part descriptors for precise manipulation in a zero-shot setting by utilizing web-trained text-to-image diffusion-based generative models. We tackle the problem by framing it as a dense semantic part correspondence task. Our model returns a gripper pose for manipulating a specific part, using as reference a user-defined click from a source image of a visually different instance of the same object. We require no manual grasping demonstrations as we leverage the intrinsic object geometry and features. Practical experiments in a real-world tabletop scenario validate the efficacy of our approach, demonstrating its potential for advancing semantic-aware robotics manipulation. Web page: https://tsagkas.github.io/click2grasp

==> sections/01_introduction.tex <==
\section{Introduction}

% General Problem Description
Developing semantics-aware manipulation pipelines, with the ability to generalize across scenes and objects, remains to this day an open research challenge. While recent approaches have predominantly concentrated on object-level manipulation, emphasizing the use of language as a communication interface between users and robots, little evidence supports the efficacy of existing methods in achieving fine-grained semantic manipulation. This gap is particularly evident in scenarios marked by pronounced visual and/or geometric ambiguity, such as distinguishing between the left and right arm of a stuffed toy or discerning the front-left from the back-right leg of a chair.

% What is the current established methodology for this problem:
In recent years, a common practice for addressing conventional robotics tasks in a zero-shot and generalisable manner has involved the fusing of features from web-trained foundation models~\cite{firoozi2023foundation} into scene representations, such as point clouds and neural fields. This approach, applicable across tasks ranging from tabletop object manipulation~\cite{shen2023F3RM,wang2023d3fields} to semantic mapping~\cite{tsagkas2023vlfields,shafiullah2023clipfields,huang2023visual,conceptgraphs}, has demonstrated considerable success. However, these features often fall short of achieving granularity finer than the object level. Strategies to overcome this limitation typically involve deploying fine-tuned versions of these models~\cite{sundaresan2023kite}, enabling the grounding of fine-grained semantic features. Nevertheless, this choice can often compromise the generalization capabilities of foundation models. Conversely, fully end-to-end frameworks~\cite{rt12022arxiv, shridhar2021cliport} are notably data-intensive, and only recently has the first extensive robotics dataset been released~\cite{embodimentcollaboration2023open}, a collaborative effort involving over 20 institutes.

% What changed that makes room for a new direction? -> SD:
Recently, diffusion models have become the prevailing choice for text-to-image generation~\cite{sd, ho2022classifierfree, nichol2022glide, ramesh2022hierarchical, saharia2022photorealistic}. Similar to prior vision model types~\cite{caron2021emerging}, an interest has been developed for utilizing the intermediate activations as representations for downstream vision tasks~\cite{couairon2022diffedit}. In particular, even in a zero-shot setting, these feature maps have led to state-of-the-art performance in the task of dense semantic correspondence~\cite{zhang2023tale,luo2023dhf,tang2023emergent}.  

% What we demonstrate in this paper:
In addressing the aforementioned manipulation-related challenges, we frame the fine-grained semantic object manipulation task as a dense semantic correspondence problem, relying on the recent advancements in the use of intermediate diffusion activations. More specifically, we develop a multi-view consistent scene representation from a two-camera setup, which we fuse with features extracted from the noising process of Stable Diffusion~\cite{sd}. Working on a real world tabletop with objects from N diverse classes, we demonstrated the benefits of this approach. 

==> sections/02_related_works.tex <==
\section{Related Work}

\noindent \textbf{Stable Diffusion for Downstream Vision Tasks}: The use of text-to-image diffusion models~\cite{sd, ho2022classifierfree, nichol2022glide, ramesh2022hierarchical, saharia2022photorealistic} has recently expanded beyond their original scope, proving successful in conventional computer vision tasks (e.g., semantic segmentation~\cite{amit2022segdiff, baranchuk2022labelefficient, chen2023generalist, jiang2018difnet, tan2023semantic, wolleb2021diffusion}). A novel approach leverages the text-conditioned Latent Diffusion Model, commonly known as Stable Diffusion (SD)~\cite{sd}, as a large pre-trained foundation model for downstream computer vision tasks. Some examples are zero-shot classification~\cite{li2023diffusion, clark2023texttoimage}, segmentation~\cite{xu2022odise, khani2023slime} and image editing~\cite{couairon2022diffedit, goel2023pair, kawar2023imagic, Tumanyan_2023_CVPR}. Notably, this strategy has demonstrated considerable success in semantic correspondence~\cite{hedlin2023unsupervised,zhang2023tale,luo2023dhf,tang2023emergent}. These methods are characterized by comparable performance in the mainstream correspondence datasets. We highlight key insights from these approaches. 

First, except for~\cite{hedlin2023unsupervised}, which utilizes activations from cross-attention operations in the U-Net layers, other works rely on the outputs of the residual block. This choice is motivated by an optimization process akin to textual inversion. In this process, an embedding $e^{*}$ is optimized to condition SD so that the cross-attention feature maps exhibit the highest activations at the corresponding area. Second, there is a distinction regarding the need for further optimization. In~\cite{zhang2023tale,luo2023dhf,tang2023emergent}, the intermediate U-Net features suffice to surpass prior arts in the task, whereas~\cite{hedlin2023unsupervised} requires the optimization of this conditioning embedding. Third, although all aforementioned SD-based methods rely on the denoising (generation) process,~\cite{luo2023dhf} reveals that the noising (inversion) process actually retains crucial semantic visual information. Finally, the complementary nature of SD and DINO features was highlighted in~\cite{zhang2023tale}, further enhancing performance in semantic correspondence. In our work, we integrate findings from~\cite{zhang2023tale} and~\cite{luo2023dhf}, combining feature maps from the inverse process of SD with those from DINOv2, for developing visual descriptors.\newline

% In X, the cross-attention layer is utilized, in Y plug-nplay the self-attention and resblock featrues, while in most of the dsc works, the output features of the resblocks are utilized in the decoder part of the UNet. 

% \noindent \textbf{Visual Foundation Models}: In general, 
% the term ``foundation model'' typically refers to large-scale, web-trained machine learning models, which can be deployed in downstream tasks directly or after fine-tuning. 



\noindent \textbf{Dense Visual Descriptors for Manipulation}: Learning robust, dense visual descriptors, adaptable to varying viewing conditions and applicable across diverse instances of object classes, has long been integral to the field of manipulation~\cite{sundaresan2020learning,ganapathi2020learning,manuelli2020keypoints,florence2019selfsupervised,pmlr-v87-florence18a, nerf-supervision}. However, the rise of large, web-trained foundation models, has highlighted the efficacy of embeddings derived from self-supervised models like DINO~\cite{caron2021emerging,oquab2023dinov2} or CLIP~\cite{radford2021learning}, offering rich semantic representations at the object level. The quality of these features can be enhanced by fusing and combining the predicted embeddings into spatial representations, leveraging the diversity of views that reveal distinct object facets. In F3RM~\cite{shen2023F3RM}, DINO or CLIP features are distilled into a neural field, with 3D descriptors obtained via demonstrations, by querying the implicit function in 3D coordinates sampled from a Gaussian distribution at the point of interaction. However, this scheme necessitates dense views and entails time-consuming re-training following scene changes. In D$^3$Fields~\cite{wang2023d3fields}, a dynamic representation is introduced, leveraging four camera views. Features from DINO, Grounded-DINO, SAM and X-Mem are employed for extracting and tracking descriptors, crucial for learning the object dynamics. Nonetheless, it remains unclear whether the extracted descriptors from such scene representations encode fine-grained semantics. Recently, this problem was addressed in LERF-TOGO~\cite{rashid2023language} for targeting specific parts of objects for interaction, however, disambiguating between geometrically and visually similar object parts remains to this day an open challenge.\newline

\noindent \textbf{Fine-Grained Semantic Object Manipulation}: Training models that can interact with objects in a specific way (e.g., grasping a stuffed toy from the left ear) is a longstanding problem in the robotics. Relevant works: KITE, CLIPort, RT-1, SayCan, etc. In VOxPoser, fine-graiend interaction is treated as a high-level planing problem via LLMs (code as policy). In KITE~\cite{sundaresan2023kite}, a fine-tuned VLM was adopted from~\cite{shridhar2021cliport} and slightly addressed our problem our hand, by being able to identify fine-grained semantics concepts. Nevertheless, our goal is to solve the problem in a zero-shot manner. These approaches have the benefit that connect manipulation with natural language and in some cases, a certain skill is learned via a significant number of demonstrations. However, relying on demonstrations is extremely time-consuming. On the other hand, 2D visual foundation models have demonstrated positive results in this direction, as was presented in section X. Consequently, we argue that for simple pick and place tasks, fine-grained semantic manipulation can be achieved by simply 3D lifting these features, and interacting with the objects in a simple gripper constrained optimization.   






 










==> sections/03_problem_formulation.tex <==
\section{Problem Formulation}

\begin{itemize}
    \item How do we deploy SD?
    \item How do we Use DINO?
    
\end{itemize}

We follow a process similar to X, making calls to the UNet componet of SD

==> sections/04_where_to_grasp.tex <==
\section{W2G: Where to grasp?}
In this segment, we introduce the overall methodology of our approach. We start by summarizing the problem at hand in Section \ref{ssec:problem_formulation}. In Section \ref{ssec:descriptors} we present the process of extracting features from foundation models and their accumulation into semantically rich visual descriptors. Afterwards, in Section \ref{ssec:scene_representation} the development of a scene representation in discussed, and finally, the optimization of the robot's 6-DoF gripper pose is explained in Section \ref{ssec:gripper}.


\subsection{Problem Formulation}
\label{ssec:problem_formulation}
Given an RGB image $\mathcal{I}\in\mathbb{R}^{H\times W \times 3}$, depicting any instance of an object class, and a user defined 2D coordinates $(u,v)$ in the pixel space, indicating a targeted area of interaction, our goal is to pick-and-place any object of that object class in the real world, from the designated area of interaction, without relying on demonstrations, in a zero-shot manner.

To achieve this, we first generate a descriptor of the designated interaction area. First, the $(u,v)$ fed along with the image $\mathcal{I}$ into a general purpose segmentation model~\cite{X} to extract a mask of the area (e.g., if the coordinates fall on a stuffed-toys arm, the mask of that arm is extracted). Then the image is fed to the visual foundation models to extract feature maps. The embeddings from the corresponding area of the mask are averaged, generating a descriptor of our interaction area. 

We consider available a setup with two RGB-D calibrated cameras, a robot arm and a tabletop with the object that is to be picked. Our overall pipeline consists of developing a scene representation in the form of an implicit function, which fuses from the different views feature-maps from large pre-trained foundation models. 


\subsection{Fine-Grained Semantic Diffusion Descriptors}
\label{ssec:descriptors}

\subsection{Scene Representation}
\label{ssec:scene_representation}
\begin{itemize}
    \item How do we deploy SD?
    \item How do we Use DINO?
\end{itemize}
We follow a process similar to X, making calls to the UNet componet of SD

\subsection{Gripper Pose Optimization}
\label{ssec:gripper}

% Notation 
For the purpose of interacting with an object in the targeted area, we optimize the transformation $\textbf{T} \in \mathbb{SE}(3)$ to be applied on the robot's end effector, for determining its final 6-DoF pose in the world coordinate system, where $\mathbb{SE}(3) = \{ (\textbf{R}, \textbf{t}) \,|\, \textbf{R} \in \mathbb{SO}(3),\, \textbf{t} \in \mathbb{R}^3 \}$ and $\textbf{R}$ and $\textbf{t}$ are the rotation matrix and translation vector, respectively. Our approach is similar to~\cite{shen2023F3RM}, however, we do not require any kind of manipulation demonstrations to optimize the pose. Instead, we rely on the gripper's and scene geometry to guide the transformation to a collision free solution. We also find that regularizing the $\textbf{R}$, $\textbf{t}$ values stabilizes the process. 

% Initializing poses
Given the implicit nature of our representation, we convert it into a voxel grid, spanning a volume $H_t \times W_t \times L_t$ over the tabletop, with voxel size equal to $\delta$. After initializing the grid, we query $\mathcal{F}$ and assign to each voxel a feature embedding. To localize the targeted area of interaction, we set a similarity threshold $t_{\text{sim}}$ and filter out the voxels with cosine similarity between their embedding and the descriptor $\textbf{f}_t$ smaller than $t_{\text{sim}}$. Then, we initialize transforms $\mathcal{T}(\textbf{R}, \textbf{t})=\{\textbf{T}\}$, by setting as $\textbf{t}$ the coordinates of the selected voxels, with random rotation matrices. 

% Subsequently, we spawn a point cloud between the fingers of the gripper that acts as a sampler of the implicit function at the area of interaction. 
% we use an elongated Gaussian with covariance $\Sigma$ and mean $\mu$ the center between the fingers of the gripper, to generate a point cloud $\mathcal{X}$. 

% Pose optimization
The center point between the gripper fingers is then utilized as the mean $\mu$ of a 3D Gaussian distribution for sampling a set of M points $\mathcal{X}_s$, that acts as a sampler of the implicit function at the area of interaction. Also, we generate another point cloud $\mathcal{X}_g$, which corresponds to the gripper's geometry, for the purpose of detecting collisions. We then leverage the differentiable nature of the implicit function $\mathcal{F}$ to compute gradients for our optimizer when querying with the transformed points of $\mathcal{X}_s$ and $\mathcal{X}_g$. Thus, we add two components to our cost function, an attractive force, guided by the features at $\textbf{T}\mathcal{X}_s$, and a repulsive force guided by the gripper geometry $\textbf{T}\mathcal{X}_g$. 

For a given visual descriptor $\textbf{f}_t$, representing the fine-grained semantics of an object type, we optimize the rotation $R$ and translation of the robot's gripper, using the ADAM optimizer~\cite{kingma2017adam}:

% \begin{equation}
%   \label{eq:optimizer}
%   \begin{aligned}
%   \mathcal{J}_{\text{pose}}(\textbf{T}; \textbf{f}_t) =
%   -\frac{1}{M} \sum_{\textbf{x}_s\in\mathcal{X}_s\mathbf{T}, \textbf{x}_g\in\mathcal{X}_g\mathbf{T}} \left(\lambda_{\text{a}} \mathcal{L}_a(\textbf{x}, \textbf{f}_t) + \lambda_{\text{r}} \mathcal{L}_r(\textbf{x})\right) + \lambda_{\text{reg}}  \mathcal{L}_{\text{reg}}(\textbf{T}),
%   \end{aligned}
% \end{equation}

\begin{equation}
  \label{eq:optimizer}
  \begin{aligned}
  \mathcal{J}_{\text{pose}}(\textbf{T}; \textbf{f}_t) =
  &-\frac{1}{M_s} \sum_{\textbf{x}_s\in\mathbf{T}\mathcal{X}_s} \lambda_{\text{a}} \mathcal{L}_a(\textbf{x}_s, \textbf{f}_t) \\ &-\frac{1}{M_g} \sum_{ \textbf{x}_g\in\mathbf{T}\mathcal{X}_g} \lambda_{\text{r}} \mathcal{L}_r(\textbf{x}_g) + \lambda_{\text{reg}}  \mathcal{L}_{\text{reg}}(\textbf{T}),
  \end{aligned}
\end{equation}


%\left( \right)
\noindent where the first two terms correspond to an attraction and a repulsion force, respectively:

\begin{equation}
   \mathcal{L}_a(\textbf{x}, \textbf{f}_t) = \frac{\mathcal{F}_f(\textbf{x}) \cdot \textbf{f}_t}{\|\mathcal{F}_f(\textbf{x})\| \cdot \|\textbf{f}_t\|},
    \mathcal{L}_r(\textbf{x}) = \mathcal{F}_d(\textbf{x})  
\end{equation}

More specifically, the $\mathcal{L}_a(\textbf{x}, \textbf{f}_t)$ term attracts the interaction area of the gripper towards points of the scene that maximize the cosine similarity between their corresponding features with the descriptor, while $\mathcal{L}_r(\textbf{x})$, pushes the entire gripper away from the scene geometry by maximizing the signed distance. The equilibrium of these forces is a collision-free gripper pose that can interact successfully with the targeted location. We also add a regularizer term: 
\begin{equation}
    \mathcal{L}_{\text{reg}}(\textbf{T}) = \|\text{\textbf{R}}\|_2 + \|\text{\textbf{t}}\|_2,
\end{equation}
\noindent which pushes the values of the rotation and translation matrices to remain low, thus further stabilizing the optimization. We repeat this optimization for all initial poses for $N_{\text{iters}}$ iterations and select the one with the lowest final cost.




==> sections/05_experiments.tex <==
\section{Experiments}

\subsection{Setup}

\subsection{Data \& 2D Evaluation}

\subsection{3D Descriptor Extraction}

\subsection{Tabletop Manipulation}

==> sections/06_results.tex <==
\section{Results}

\subsection{Manipulation Results}
Remember to mention 3 types of failure:
\begin{enumerate}
    \item object failure (I asked teddy bear and interacted with mug);
    \item semantic failure (I asked left and right was detected);
    \item Successful, localization but gripper eiter slipped or did not grasp succesfully; 
\end{enumerate}

==> sections/07_conclusion.tex <==
\section{Conclusion}

\noindent Limitations and Future Work:
\begin{itemize}
    \item We do not utilize the text to image capabilities of SD. In the future, we aim to rely on this aspect to make a common interface between descriptors and language for open-vocabulary manipulation.
\end{itemize}

==> sections/08_acknowledgment.tex <==
\section*{Acknowledgment}

